Multimodal Fusion of EHR in Structures and Semantics: Integrating Clinical Records and Notes with Hypergraph and LLM

Electronic Health Records (EHRs) have become increasingly popular to support clinical decision-making and healthcare in recent decades. EHRs usually contain heterogeneous information, such as structural data in tabular form and unstructured data in textual notes. Different types of information in EHRs can complement each other and provide a more complete picture of the health status of a patient. While there has been a lot of research on representation learning of structured EHR data, the fusion of different types of EHR data (multimodal fusion) is not well studied. This is mostly because of the complex medical coding systems used and the noise and redundancy present in the written notes. In this work, we propose a new framework called MINGLE, which integrates both structures and semantics in EHR effectively. Our framework uses a two-level infusion strategy to combine medical concept semantics and clinical note semantics into hypergraph neural networks, which learn the complex interactions between different types of data to generate visit representations for downstream prediction. Experiment results on two EHR datasets, the public MIMIC-III and private CRADLE, show that MINGLE can effectively improve predictive performance by 11.83% relatively, enhancing semantic integration as well as multimodal fusion for structural and textual EHR data.

==> Fig-ablation.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.5ex}
    \subfloat[Study of Retrievers]{
        \includegraphics[width=0.325\linewidth]{figures/dr_models.pdf}
        \label{fig:dr_models}
    } %\hfill
        \hspace{-1.5ex}
    \subfloat[Study on $k$]{
        \includegraphics[width=0.325\linewidth]{figures/para_k.pdf}
        \label{fig:para_k}
    }
    \hspace{-1.5ex}
    \subfloat[Study on $\gamma$]{
        \includegraphics[width=0.325\linewidth]{figures/para_gamma.pdf}
        \label{fig:para_gamma}
    }
    \vspace{-0.5ex}
    \caption{Studies of Different Retrieval Models and Hyperparameters (Best View in Colors).}
    \vspace{-1ex}
\label{fig:dr_model}
\end{figure}

\begin{figure}[t]
    \centering
    \vspace{-1.5ex}
    \subfloat[Pseudo Label Accuracy]{
        \includegraphics[width=0.47\linewidth]{figures/local_global_acc.pdf}
        \label{fig:local_global_acc}
    } %\hfill
         \hspace{-1ex}
    \subfloat[Macro-F1 Score]{
        \includegraphics[width=0.47\linewidth]{figures/local_global_f1.pdf}
        \label{fig:local_global_f1}
    }
    \caption{Study on Effects of Local and Global Information.}
    \vspace{-1ex}
\label{fig:local_global}
\end{figure}


% \begin{figure}[!t]
%     \centering
%     \vspace{-1.5ex}
%     \subfloat[MeSH]{
%         \includegraphics[width=0.45\linewidth]{figures/precision_recall.pdf}
%         \label{fig:mesh_dr}
%     } %\hfill
%          \hspace{-1ex}
%     \subfloat[arXiv-CS]{
%         \includegraphics[width=0.45\linewidth]{figures/mesh_recall.pdf}
%         \label{fig:arxiv_cs_dr}
%     }
%     \vspace{-1ex}
%     \caption{Hyperparameter Studies.}
%     \vspace{-0.5ex}
% \label{fig:parameter}
% \end{figure}

==> Tab-case.tex <==
\begin{table}[!t]
    \centering
     \caption{Case Study on expanded keywords for three tasks.}
    \renewcommand\arraystretch{0.9}
\resizebox{1.01\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
    \bf Dataset & \bf Class &\bf  Expanded Keyword  \\\midrule
    MeSH & Diabetes  & insulin, glucose, diabetic, metformin, glycemic\\
    MeSH & Mental Disorders  & depression, anxiety, antidepressant, schizophrenia, mood \\ %\midrule
    MeSH & Neoplasms  & tumor, carcinoma, cell, tumour, chemotherapy\\\midrule
    arXiv-Math & Combinatorics & graph, combinatorial, vertex, edge,  bipartite \\
    arXiv-Math & Number theory &  prime, integer, modulo, odd, divisor \\
    arXiv-Math & Statistics theory & estimation, sample, regression, treatment, inference \\ \midrule
    arXiv-CS & Information theory & entropy, channel, shannon, capacity, decoder \\
    arXiv-CS & Machine Learning & classifier, classification, boosting, ensemble, tree \\
    arXiv-CS & Game Theory  & player, equilibrium, nash, payoff, strategy \\
    \bottomrule
\end{tabular}}
\label{tab:case}
\end{table}

==> Tab-label-name.tex <==
\begin{table*}[!t]
    \centering
     \vspace{-1ex}
     \caption{Label Name Information. Label names in \blue{blue} never appear in the corpus.}
     \vspace{-1ex}
    \renewcommand\arraystretch{0.9}
\resizebox{\linewidth}{!}{
\begin{tabular}{cl}
\toprule
    \bf Dataset & \bf Label Names   \\\midrule
    \multirow{2}{*}{\bf MeSH} & 	 Cardiovascular diseases,  Chronic kidney disease, HIV/AIDS, Diabetes (mellitus), \blue{Chronic respiratory diseases}, \blue{Digestive diseases}, \blue{Hepatitis A/B/C/E},  \\
    &    Mental disorders,  Musculoskeletal disorders, \blue{Neoplasms (cancer)}, Neurological disorders	 \\ \midrule
    \multirow{2}{*}{\bf arXiv-Math} & Numerical Analysis,  Algebraic Geometry, Functional spaces, Number Theory,  Complex Variable
, Differential Geometry, Combinatorics, Operator Algebra,  \\
&  Representation Theory, \blue{Statistics Theory}, \blue{Topological Geometry}, Rings and Algebra, Probability
, Dynamical System, \blue{Optimization and Control}, Logic \\\midrule
    \multirow{4}{*}{\bf arXiv-CS} & Database, Computation and Language, Information Theory, Computational Geometry,  \blue{Cryptography and Security}, \blue{System and Control}, Game Theory,   \\
& \blue{Data Structures and Algorithm}, Human-Computer Interaction, Machine Learning, Information Retrieval, Programming Languages,  Software Engineering, \\
&  \blue{Networking and Internet Architecture}, Artificial Intelligence, Social and Information Networks,  Distributed, Parallel, and Cluster Computing, Robotics,  \\ & Computer Vision and Pattern Recognition, \blue{Logic in Computer Science}\\
    \bottomrule
\end{tabular}}
% \vspace{-1ex}
\label{tab:label_name}
\end{table*}
